Multi-Dimensional Balanced Graph Partitioning via Projected Gradient Descent

Motivated by performance optimization of large-scale graph processing systems that distribute the graph across multiple machines, we consider the balanced graph partitioning problem. Compared to the previous work, we study the multi-dimensional variant when balance according to multiple weight functions is required. As we demonstrate by experimental evaluation, such multi-dimensional balance is important for achieving performance improvements for typical distributed graph processing workloads. We propose a new scalable technique for the multidimensional balanced graph partitioning problem. The method is based on applying randomized projected gradient descent to a non-convex continuous relaxation of the objective. We show how to implement the new algorithm efficiently in both theory and practice utilizing various approaches for projection. Experiments with large-scale social networks containing up to hundreds of billions of edges indicate that our algorithm has superior performance compared with the state-of-the-art approaches.

==> convergence.tex <==
\section{Towards convergence analysis}\label{app:convergence}
%If the domain of $f$ is restricted to $[-\Delta, \Delta]^{|V|}$ then the Lipschitz constant of $f \colon [-\Delta, \Delta]^{|V|} \to \mathbb R$ is:
%$$K = \sup_{\vx \in [-\Delta,\Delta]^{|V|}} \|\nabla f(\vx)\|_2 \le \Delta d \sqrt{|V|},$$
%where $d$ is the maximum degree in $G$.




\begin{lemma}[Bertsekas, Section 2.3.2]\label{lem:pgd-step}
	If $\|\nabla f(\vx) - \nabla f(\vy)\| \le L \|\vx - \vy\|$ for all $\vx, \vy \in \mathbb R^n$ and $0 < \gamma < 2/L$ then 
	\begin{align*}
	f(\vx_{t + 1}) - f(\vx_t) \ge \left(\frac{1}{\gamma} - \frac{L}{2}\right)\|\vx_t - \vx_{t+1}\|_2^2
	\end{align*}
	
\end{lemma}

\begin{proof}
	
	We use the following Descent Lemma:
	
	\begin{proposition}[Descent Lemma]
		Let $f \colon \mathbb R^n \to \mathbb R$ be continuously differentiable, and let $\vx$ and $\vy$ be two vectors in $\mathbb R^n$. If for all $t \in [0,1]$ it holds that $\|\nabla f(\vx + t\vy) - \nabla f(\vx)\| \le L t \|\vy\|$ where $L$ is a constant then:
		$$f(\vx + \vy) \ge f(\vx) + \vy^T \nabla f(\vx) - \frac{L}{2} \|\vy\|_2^2$$
	\end{proposition}
	\begin{proof}
		Let $t$ be a scalar and let $g(t) = f(\vx + t \vy)$. By the chain rule $(d g / dt)(t) = \vy^T \nabla f(\vx + t\vy)$.
		Then:
		\begin{align*}
		f(\vx + \vy) - f(\vx) &= g(1) - g(0) \\
		& = \int_0^1 \frac{d g}{d t}(g) dt \\
		& = \int_0^1 \vy^T \nabla f(\vx + t \vy) dt \\
		&\ge \int_0^1 \vy^T \nabla f(\vx) dt - \left|\int_0^1 \vy^T (\nabla f(\vx + t \vy) - \nabla f(\vx)) dt\right| \\
		&\ge \int_0^1 \vy^T \nabla f(\vx) dt  - \int_0^1 \|\vy\|_2 \|\nabla f(\vx + t \vy) - \nabla f(\vx)\|_2dt\\
		& \ge \vy^T \nabla f(\vx) - \|\vy\|_2 \int_0^1 L t \|\vy\|_2 dt \\
		& = \vy^T \nabla f(\vx) - \frac{L}{2} \|\vy\|_2^2
		\end{align*}
	\end{proof}
	
	
	By the Descent Lemma we have:
	\begin{align*}
	f(\vx_{t + 1}) - f(\vx_t) \ge \nabla f(\vx_t)(\vx_{t + 1} - \vx_t) - \frac{L}{2}\|\vx_{t + 1} - \vx_t\|_2^2.
	\end{align*}
	
	Note that since $K = \mathcal S_0 \cap \mathcal B_\infty$ is a convex body and $\vx_{t + 1}$ is a projection of $\vy_{t + 1}$ on $K$ for every $\vx \in K$ it holds that:
	$$(\vy_{t + 1} - \vx_{t + 1})(\vx - \vx_{t + 1}) \le 0.$$
	Applying this to $\vx = \vx_t$ and using the fact that $\vy_{t + 1} = \vx_t + \gamma \nabla f(\vx_t)$ we have:
	$$(\vx_t + \gamma \nabla f(\vx_t) - \vx_{t + 1})(\vx_t - \vx_{t + 1}) \le 0,$$
	which implies that $\nabla f(\vx_t) (\vx_{t+1} - \vx_{t}) \ge \frac{1}{\gamma}\|\vx_t - \vx_{t+1}\|_2^2$. Hence we have:
	\begin{align*}
	f(\vx_{k + 1}) - f(\vx_k) \ge \left(\frac{1}{\gamma} - \frac{L}{2}\right)\|\vx_t - \vx_{t+1}\|_2^2
	\end{align*}
	
	%\textbf{The part below I don't quite understand, I think something is missing.}
	%Thus if $\gamma < 2/L$, the RHS of the above is nonnegative so if $\{\vx_t\}$ has a limit point the LHS tends to $0$.
	%Therefore, $\|\vx_{t + 1} - \vx_t\| \to 0$, which implies that for every limit point $\bar \vx$ of $\{\vx_t\}$ we have $[\bar \vx + \gamma \nabla f(\bar \vx)]^+ = \bar \vx$, so $\bar \vx$ is stationary (here we use notation $[\vx]^+$ to denote the projection of a vector $\vx$ on $K$).
\end{proof}

\subsection{First step}


Let's analyze the first step. We show the following theorem:
\begin{theorem}
	Let $\lambda_{max} = \max(|\lambda_1|, |\lambda_n|)$ then
	if $\gamma = 1/\lambda_{max}$ then $\mathbb E[f(\vx_1)] \ge \frac{\eta^2 |E|}{2 \lambda_{max}}$ (assuming we don't have to round the coordinates\gtodo{Fix this!}).
\end{theorem}

Recall that we set $\vx_0 = 0^n$ and consider three points $\vx_0', \vx_1$ and $\vy_1$. These three points lie in a hyperplane $H'$ which is orthogonal to the hyperplane $H = \{\vx \colon \langle \vone, \vx \rangle = 0\}$, where $\vone = (\frac{1}{\sqrt{n}}, \dots, \frac{1}{\sqrt{n}})$.
Let $\vx_0''$ be the projection of $\vx_0'$ on $H$.
Then $\vx_0''$ also lies in $H'$.

We have $\|\vx_1 - \vx_0'\|_2^2 = \|\vx_0' - \vx''_0\|_2^2 + \|\vx_0'' - \vx_1\|_2^2$.
Let $\vy_1'$ be the projection of $\vx_0'$ on the line through $\vy_1$ and $\vx_1$.
Then $\|\vx_0' - \vy_1\|_2^2 = \|\vx_0' - \vy_1'\|_2^2 + \|\vy_1' - \vy_1\|_2^2$.
Since $\|\vx_0' - \vy_1'\|_2^2 = \|\vx_0'' - \vx_1\|_2^2$ we have:
\begin{align*}
\|\vx_1 - \vx_0'\|_2^2 = \|\vx_0' - \vx_0''\|_2^2 + \|\vx_0' - \vy_1\|_2^2 - \|\vy_1' - \vy_1\|_2^2.
\end{align*}

We now take expectations and make use of the Lemma~\ref{lem:first-pgd-step-geometry} which is proved below:
\begin{align*}
\mathbb E\left[\|\vx_1 - \vx_0'\|_2^2\right] &= \eta^2 \left(1 + \gamma^2 \|A\|_F^2 - \gamma^2 \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i\rangle^2\right) \\
& \ge \eta^2 (1 + 2 \gamma^2 |E| - \gamma^2 \max(\lambda_1^2, \lambda_n^2))
\end{align*}

%The following is a standard fact about eigenvalues of the adjacency matrix (see e.g. Lovasz\gtodo{add citation}):
%\begin{proposition}
%If $\bar d = \frac{1}{n} \sum_{i = 1}^n d_i$ is the average degree and $\lambda_1$ is the largest eigenvalue of the adjacency matrix then:
%$$\max(\bar d,\sqrt{d_{max}})\le \lambda_1 \le d_{max}$$
%\end{proposition}
%
%Hence:
%\begin{align*}
%\mathbb E\left[\|\vx_1 - \vx_0'\|_2^2\right] \ge \eta^2 (1 + \gamma^2 (|E| - d_{max}^2) )
%\end{align*}

By Lemma~\ref{lem:pgd-step} using the fact that for our function $f(\vx) = \vx^T A \vx$ we have $L \le \max(|\lambda_1|, |\lambda_n|)$ we obtain:
$$f(\vx_1) - f(\vx_0') \ge \left(\frac{1}{\gamma} - \frac{\max( |\lambda_1|, |\lambda_n|)}{2}\right) \|\vx_1 - \vx_0'\|_2^2.$$

Setting $\gamma = 1/ \max(|\lambda_1|, |\lambda_n|)$ and taking expectations we have:
$$\mathbb E[f(\vx_1) - f(\vx_0')] \ge \frac{\eta^2|E|}{2 \max(|\lambda_1|, |\lambda_n|)}  $$

Finally note that:
$$\mathbb E[f(\vx_0')] = \mathbb E[\vx_0' A \vx_0'] = \eta^2 \sum_{i = 1}^n \lambda_i = \eta^2 tr(A) = 0,$$
and hence the proof of the theorem follows.

It remains to prove Lemma~\ref{lem:first-pgd-step-geometry}.

\begin{lemma}\label{lem:first-pgd-step-geometry}
	If $A = \sum_{i = 1}^n \lambda_i v_i v_i^T$ is the eigendecomposition of $A$ where $v_i$'s form an orthonormal basis then:
	\begin{align*}
	&\mathbb E[\|\vx_0' - \vx_0''\|_2^2] = \eta^2 \\
	&\mathbb E[\|\vx_0' - \vy_1\|_2^2 ] = \eta^2 \gamma^2 \|A\|_F^2\\
	&\mathbb E[\|\vy_1' - \vy_1\|_2^2] = \eta^2 \gamma^2 \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i \rangle^2
	\end{align*}
\end{lemma}
\begin{proof}
	We have $\mathbb E[\|\vx_0' - \vx_0''\|_2^2] = \mathbb E[\langle \vone, \vx_0' \rangle^2]ß = \eta^2$, where the second equality follows by rotational symmetry of the Gaussian distribution. 
	
	%$$\mathbb E[(\sum_{i = 1}^n \frac{1}{\sqrt n} (\vx_0')_i)^2] = \frac{1}{n} \mathbb E[\sum_{i = 1}^n (\vx_0')_i^2] = \eta^2 $$
	
	We have: 
	\begin{align*}
	\mathbb E[\|\vx_0' - \vy_1\|_2^2] &= \mathbb E[\|\gamma A \vx_0'\|_2^2] \\
	&= \mathbb E\left[\gamma^2 \vx_0'^T A^2 \vx_0' \right]\\
	&= \mathbb E\left[\gamma^2 \vx_0'^T \left(\sum_{i = 1}^n \lambda^2_i v_i v_i^T\right) \vx_0' \right]\\
	&= \gamma^2 \sum_{i = 1}^n \lambda^2_i \mathbb E\left[\langle v_i, \vx_0'\rangle^2\right] \\
	&= \gamma^2 \eta^2 \|A\|_F^2,
	\end{align*}
	where in the last equality we use the fact that since each $v_i$ is a unit vector $\mathbb E[\langle v_i, \vx_0'\rangle ] = \eta^2$ by the rotational symmetry of the Gaussian distribution.
	
	Finally, we have:
	\begin{align*}
	\mathbb E[\|\vy_1' - \vy_1\|_2^2] &= \mathbb E[\langle \vone, \vy_1 - \vx_0' \rangle^2 ] \\
	&= \mathbb E[\langle \vone, \gamma A \vx_0' \rangle^2] \\
	&= \gamma^2 \mathbb E\left[\left(\vone^T \left(\sum_{i = 1}^n \lambda_i v_i v_i^T\right) \vx_0'\right)^2\right] \\
	&= \gamma^2 \mathbb E\left[ \left(\sum_{i = 1}^n \lambda_i \langle\vone, v_i\rangle \langle v_i, \vx_0'\rangle \right)^2 \right] \\
	&= \gamma^2 \left(\sum_{i = 1}^n \sum_{j = 1}^n\lambda_i \lambda_j \langle\vone, v_i\rangle \langle \vone, v_j\rangle \mathbb E\left[\langle v_i, \vx_0'\rangle \langle v_j, \vx_0'\rangle\right]\right)
	\end{align*}
	Note that since $v_i$ and $v_j$ are orthogonal for $i \neq j$ we have $\mathbb E\left[\langle v_i, \vx_0'\rangle \langle v_j, \vx_0'\rangle\right] = 0$. For $i = j$ we have $\mathbb E[\langle v_i, \vx_0'\rangle^2] = \eta^2$ as before. Hence we have:
	\begin{align*}
	\mathbb E[\|\vy_1' - \vy_1\|_2^2] = \eta^2 \gamma^2 \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i \rangle^2
	\end{align*}
	
	
\end{proof}


\subsection{$t$-th step}

We will assume that noise is added in every step, i.e. the algorithm at every step looks as follows:
\begin{enumerate}
	\item Given input $\vx_t$ from the previous step let $\vx_t' = \vx_t + \eta N_n(0,1)$.
	\item Let $\vy_{t + 1} = \vx_t' + \gamma A \vx_t'$
	\item Set $\vx_{t + 1} = \arg min_{\vx \in \mathcal S_0 \cap \mathcal B_\infty} \|\vy_{t + 1} - \vx\|$.
\end{enumerate}

We need an analog of Lemma~\ref{lem:first-pgd-step-geometry}.
\begin{lemma}
	\begin{align*}
%	\mathbb E[\|\vx_t' - \vx_t''\|_2^2] = \eta^2 \\
	\mathbb E[\|\vy_{t + 1} - \vx_{t}'\|_2^2] - \mathbb E[\|\vy_{t + 1}' - \vy_{t + 1}\|_2^2] \ge \gamma^2 \eta^2 \left(\|A\|_F^2 - \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i \rangle^2\right)
	\end{align*}
\end{lemma}
\begin{proof}
	Let $\vz \sim N_n(0,1)$. Then for the first term we have:
	\begin{align*}
	\mathbb E[\|\vy_{t + 1} - \vx_{t}'\|_2^2] &= \mathbb E[\|\gamma A \vx_t'\|_2^2] \\ 
	&= \gamma^2 \mathbb E[\vx_t'^T A^2 \vx_t'] \\
	&= \gamma^2 \mathbb E[(\vx_t + \eta \vz)^T A^2 (\vx_t + \eta \vz)] \\
	& = \gamma^2 \left(\vx_t^T A^2 \vx_t + 2 \eta \mathbb E[\vz^T A^2 \vx_t] + \eta^2 \mathbb E[\vz^T A^2 \vz]\right)
	\end{align*}
	We have $\mathbb E[\mathbb \vz^T A^2 \vz] = \|A\|_F^2$ as in the proof of Lemma~\ref{lem:first-pgd-step-geometry}.
	Furthermore, $\mathbb E[\vz^T A^2 \vx_t] = \mathbb E[\langle \vz, A^2 \vx_t\rangle] = 0$ where the second equality follows by the linearity of expectation using the fact that $\mathbb E[\vz_i] = 0$ for each $i$.
	We have $\vx_t^T A^2 \vx_t = \sum_{i = 1}^n \lambda_i^2 \langle v_i, \vx_t\rangle^2$ and hence:
	$$\mathbb E[\|\vy_{t + 1} - \vx_{t}'\|_2^2] =\gamma^2 \eta^2 \|A\|_F^2 + \gamma^2 \sum_{i = 1}^n \lambda_i^2 \langle v_i, \vx_t\rangle^2$$

	We have:
	\begin{align*}
	\mathbb E[\|\vy_{t + 1}' - \vy_{t + 1}\|_2^2] &= \mathbb E[\langle \vone, \vy_{t + 1} - \vx_t' \rangle^2 ] \\
	&= \mathbb E[\langle \vone, \gamma A \vx_t' \rangle^2] \\
	&= \gamma^2 \mathbb E\left[\left(\vone^T \left(\sum_{i = 1}^n \lambda_i v_i v_i^T\right) \vx_t'\right)^2\right] \\
	&= \gamma^2 \mathbb E\left[ \left(\sum_{i = 1}^n \lambda_i \langle\vone, v_i\rangle \langle v_i, \vx_t + \eta \vz \rangle \right)^2 \right] \\
	&= \gamma^2 \left(\sum_{i = 1}^n \sum_{j = 1}^n\lambda_i \lambda_j \langle\vone, v_i\rangle \langle \vone, v_j\rangle \mathbb E\left[\langle v_i, \vx_t + \eta \vz \rangle \langle v_j, \vx_t + \eta \vz \rangle\right]\right)
	\end{align*}
	
	We have:
	\begin{align*}
	\mathbb E\left[\langle v_i, \vx_t + \eta \vz \rangle \langle v_j, \vx_t + \eta \vz \rangle\right] &= \langle v_i, \vx_t \rangle \langle v_j, \vx_t \rangle + \mathbb E[\langle v_i, \eta \vz \rangle] + \mathbb E[\langle v_j, \eta \vz\rangle] + \eta^2 \mathbb E[\langle v_i, \vz \rangle \langle v_j, \vz \rangle]\\
	&= \langle v_i, \vx_t \rangle \langle v_j, \vx_t \rangle + \eta^2 \delta_{ij}
	\end{align*}
	and hence:
	\begin{align*}
	\mathbb E[\|\vy_{t + 1}' - \vy_{t + 1}\|_2^2] = \gamma^2 \left(\sum_{i = 1}^n \sum_{j = 1}^n \lambda_i \lambda_j \langle \vone, v_i \rangle \langle \vone, v_j \rangle \langle v_i, \vx_t \rangle \langle v_j, \vx_t \rangle + \eta^2 \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i \rangle^2\right)
	\end{align*}

Consider the difference $\mathbb E[\|\vy_{t + 1} - \vx_{t}'\|_2^2] - \mathbb E[\|\vy_{t + 1}' - \vy_{t + 1}\|_2^2]$. The proof follows from the following proposition:
\begin{proposition}
$$\sum_{i = 1}^n \lambda_i^2 \langle v_i, \vx_t\rangle^2 - \sum_{i = 1}^n \sum_{j = 1}^n \lambda_i \lambda_j \langle \vone, v_i \rangle \langle \vone, v_j \rangle \langle v_i, \vx_t \rangle \langle v_j, \vx_t \rangle \ge 0.$$
\end{proposition}
\begin{proof}
Let $\valpha$ be a vector with coordinates $\alpha_i = \lambda_i \langle v_i, \vx_t\rangle$ and $\vbeta$ be a vector with coordinates $\vbeta_i = \langle \vone, v_i \rangle$.
Note that $\|\vbeta\|_2^2 = 1$ since $v_i$'s form an orthonormal basis and $\vone$ is a unit vector.
Using this notation we need to show that $\|\valpha\|_2^2 - \langle \valpha, \vbeta\rangle^2 \ge 0$.
This follows from Cauchy-Schwarz since $\langle \valpha, \vbeta\rangle^2 \le \|\alpha\|_2^2 \|\vbeta\|_2^2 = \|\valpha\|_2^2$.
\end{proof}
	
%	Note that since $v_i$ and $v_j$ are orthogonal for $i \neq j$ we have $\mathbb E\left[\langle v_i, \vx_0'\rangle \langle v_j, \vx_0'\rangle\right] = 0$. For $i = j$ we have $\mathbb E[\langle v_i, \vx_0'\rangle^2] = \eta^2$ as before. Hence we have:
%	\begin{align*}
%	\mathbb E[\|\vy_1' - \vy_1\|_2^2] = \eta^2 \gamma^2 \sum_{i = 1}^n \lambda_i^2 \langle \vone, v_i \rangle^2
%	\end{align*}
	
\end{proof}	
	
\subsection{Analysis with fixed variables: first step}

Now suppose that we have some of the variables in the algorithm fixed.
By rearranging indices we have $\vx_t = (\vx_{t,r}, \vc_{t,n-r})$ where $\vx_{t,r}$ is an $r$-dimensional vector of variables and $\vc_{t,n-r} \in \{-1,1\}^{n - r}$ is a vector of fixed variables.
Similarly we can represent $A$ as a block matrix: 
\begin{align*}
A = \left[\begin{array}{cc} A_r & C_{n-r} \\ C_{n -r}^T & B_{n - r}\end{array}\right].
\end{align*}
Then the quadratic form $\vx_t^T A \vx_t$ becomes:
\begin{align*}
\vx_t^T A \vx_t &= (\vx_{t,r}, \vc_{t,n-r})^T \left[\begin{array}{cc} A_r & C_{n-r} \\ C_{n -r}^T & B_{n - r}\end{array}\right] (\vx_{t,r}, \vc_{t, n - r}) \\
&= \vx_{t,r}^T A_r \vx_{t,r} + 2 \vc_{t,n-r}^T C^T_{n-r} \vx_{t,r} + \vc_{t,n-r}^T B_{n-r} \vc_{t,n-r} 
\end{align*}
To simplify presentation we drop the second  index in all vectors in the discussion below.
Then our objective, its gradient and Hessian are given as: 
\begin{align*}
&f(\vx_t) = \vx_t^T A_r \vx_t + 2\vx_t^T C_{n - r} \vc_t   + \vc_t^T B_{n-r} \vc_t \\
&\nabla f(\vx_t) = A_r \vx_t + 2  C_{n-r} \vc_t \\
&\nabla^2 f(\vx_t) = A_r
\end{align*}
We need an analog of Lemma~\ref{lem:first-pgd-step-geometry}:
\begin{lemma}
If $A_r = \sum_{i = 1}^r \lambda_i v_i v_i^T$ is the eigendecomposition of $A_r$ where $v_i$'s form an orthonormal basis then:
\begin{align*}
%&\mathbb E[\|\vx_0' - \vx_0''\|_2^2] = \eta^2 \\
\mathbb E[\|\vx_0' - \vy_1\|_2^2 ] - \mathbb E[\|\vy_1' - \vy_1\|_2^2] = \eta^2 \gamma^2 \left(\|A_r\|_F^2 - \sum_{i = 1}^r \lambda_i^2 \langle \vone, v_i \rangle^2\right) 
\end{align*}
\end{lemma}
\begin{proof}
%	The first part is as in Lemma~\ref{lem:first-pgd-step-geometry}
For the first term we have: 
\begin{align*}
\mathbb E[\|\vx_0' - \vy_1\|_2^2] &= \mathbb E[\|\gamma (A_r \vx_0' + 2  C_{n - r}\vc_0)\|_2^2] \\
&= \mathbb E\left[\gamma^2 (A_r \vx_0' + 2  C_{n - r} \vc_0)^T(A_r \vx_0' + 2  C_{n - r} \vc_0) \right]\\
&= \gamma^2 \mathbb E\left[\vx_0'^T A_r^2 \vx_0' + 4 \vc_0^T C_{n - r}^T  A_r \vx_0' + 4\vc_0^T C_{n - r}^T C_{n -r} \vc_0\right].
%&= \mathbb E\left[\gamma^2 \vx_0'^T \left(\sum_{i = 1}^n \lambda^2_i v_i v_i^T\right) \vx_0' \right]\\
%&= \gamma^2 \sum_{i = 1}^n \lambda^2_i \mathbb E\left[\langle v_i, \vx_0'\rangle^2\right] \\
%&= \gamma^2 \eta^2 \|A\|_F^2,
\end{align*}
We have $\mathbb E[\vx_0' A^2_r \vx_0'] = \eta^2 \|A_r\|_F^2$. Denoting $C_{n-r}\vc_0$ as $\vc$ the expectation of the cross term is:
\begin{align*}
\mathbb E\left[\vc^T A_r \vx_0'\right] &= \mathbb E\left[\vc^T \left(\sum_{i = 1}^r \lambda_i v_i v_i^T\right) \vx_0'\right]\\
&= \sum_{i = 1}^r \lambda_i \langle c, v_i \rangle \mathbb E\left[\langle v_i, \vx_0 \rangle\right] \\
& = 0.
\end{align*}
Thus for the first term:
\begin{align*}
\mathbb E[\|\vx_0' - \vy_1\|_2^2] = \eta^2 \gamma^2 \|A_r\|_F^2 + 4 \gamma^2 \|\vc\|_2^2
\end{align*}

For the second term we have:
\begin{align*}
\mathbb E[\|\vy_1' - \vy_1\|_2^2] &= \mathbb E[\langle \vone, \vy_1 - \vx_0' \rangle^2 ] \\
&= \mathbb E[\langle \vone, \gamma (A_r \vx_0' + 2  C_{n-r} \vc_0) \rangle^2] \\
&= \gamma^2 \mathbb E\left[\left(\vone^T \left(\sum_{i = 1}^r \lambda_i v_i v_i^T\right) \vx_0' + 2\cdot \vone^T C_{n - r} \vc_0\right)^2\right] \\
&= \eta^2 \gamma^2 \sum_{i = 1}^r \lambda_i^2 \langle \vone, v_i \rangle^2  + 4\gamma^2\mathbb E[\vc^T A_r\vx_0'] + 4 \gamma^2 \|\vc\|_2^2\\
&= \eta^2 \gamma^2 \sum_{i = 1}^r \lambda_i^2 \langle \vone, v_i \rangle^2   + 4 \gamma^2 \|\vc\|_2^2,\\
\end{align*}
where the expectation of the cross term $\mathbb E[\vc^T A_r \vx_0']$ is zero as computed above and $\mathbb E[(\vone^T A_r \vx_0')^2]$ is computed as in the proof of Lemma~\ref{lem:first-pgd-step-geometry}.

Taking the difference between the two terms the proof follows.

\subsection{Analysis with fixed variables: $t$-th step}
We would like to show the following:
\begin{lemma}
	If $A_r = \sum_{i = 1}^r \lambda_i v_i v_i^T$ is the eigendecomposition of $A_r$ where $v_i$'s form an orthonormal basis then:
	\begin{align*}
	%&\mathbb E[\|\vx_0' - \vx_0''\|_2^2] = \eta^2 \\
	\mathbb E[\|\vx_t' - \vy_{t +1}\|_2^2 ] - \mathbb E[\|\vy_{t + 1}' - \vy_{t + 1}\|_2^2] \ge \eta^2 \gamma^2 \left(\|A_r\|_F^2 - \sum_{i = 1}^r \lambda_i^2 \langle \vone, v_i \rangle^2\right) 
	\end{align*}
\end{lemma}

Note that there might be some complications because now we are projecting not on the hyperplane orthogonal to $\vone$ as some of our variables are fixed and hence the sum shouldn't be zero but some constant. I guess, this can be fixed by just picking a different unit vector in the orthogonal direction.

\end{proof}

\subsection{Random Gaussian vs. random vector on a sphere}
It might be useful to replace random Gaussians with random vectors on a sphere so that our noise is $\eta S_n$ where $S_n$ is a random vector on a unit sphere.

In the convergence analysis we are using the following facts about random Gaussians. Let $\vz \sim N_n(0,1)$, then we need that:
\begin{enumerate}
\item $\mathbb E[\langle\vz, \vx\rangle] = 0$ for any fixed unit vector $\vx$.
\item $\mathbb E[\langle \vz, \vx \rangle^2] = \eta^2$ for any fixed unit vector $\vx$.
\item $\mathbb E[\langle \vz, \vx \rangle \langle \vz, \vy \rangle] = \mathbb E[\langle \vz, \vx \rangle] \mathbb E[\langle \vz, \vy \rangle] = 0$ for any $\vx \perp \vy$.
\end{enumerate}

Here facts 1 and 3 still hold for a scaled random vector on a unit sphere.
For fact 2 we can use the fact that $\mathbb E[\langle \vz, \vx\rangle^2] = \mathbb E[z_1^2] = 1/n$ where the the first equality follows from the symmetry of the distribution on a sphere and the second equality is since $\mathbb E[z_i^2]$ are the same for each $i$ and $\sum_{i = 1}^n z_i^2 = 1$.

==> expintro.tex <==
Our experimental results show that \algname can be scaled to graphs with up to several billions of vertices and hundreds of billions of edges and achieves similar and in many cases superior performance to the previous work, including METIS~\cite{KK95}, FENNEL~\cite{TGRV14}, Social Hash Partitioner~\cite{KKPPSAP17}, Spinner~\cite{MLLS17} and linear embedding~\cite{ABM16}.

==> instructions.tex <==
\section{Submission of papers to NIPS 2018}

NIPS requires electronic submissions.  The electronic submission site
is
\begin{center}
  \url{https://cmt.research.microsoft.com/NIPS2018/}
\end{center}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NIPS 2018 must be prepared according to the
instructions presented here. Papers may only be up to eight pages
long, including figures. Additional pages \emph{containing only
  acknowledgments and/or cited references} are allowed. Papers that
exceed eight pages of content (ignoring references) will not be
reviewed, or in any other way considered for presentation at the
conference.

The margins in 2018 are the same as since 2007, which allow for
$\sim$$15\%$ more words in the paper compared to earlier years.

Authors are required to use the NIPS \LaTeX{} style files obtainable
at the NIPS website as indicated below. Please make sure you use the
current files and not previous versions. Tweaking the style files may
be grounds for rejection.

\subsection{Retrieval of style files}

The style files for NIPS and other conference information are
available on the World Wide Web at
\begin{center}
  \url{http://www.nips.cc/}
\end{center}
The file \verb+nips_2018.pdf+ contains these instructions and
illustrates the various formatting requirements your NIPS paper must
satisfy.

The only supported style file for NIPS 2018 is \verb+nips_2018.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{}
  2.09, Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+,
which creates a camera-ready copy, \verb+preprint+, which creates a
preprint for submission to, e.g., arXiv, and \verb+nonatbib+, which will
not load the \verb+natbib+ package for you in case of package clash.

\paragraph{New preprint option for 2018}
If you wish to post a preprint of your work online, e.g., on arXiv,
using the NIPS style, please use the \verb+preprint+ option. This will
create a nonanonymized version of your work with the text
``Preprint. Work in progress.''  in the footer. This version may be
distributed as you see fit. Please \textbf{do not} use the
\verb+final+ option, which should \textbf{only} be used for papers
accepted to NIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper
as they will be removed during generation of camera-ready copies.

The file \verb+nips_2018.tex+ may be used as a ``shell'' for writing
your paper. All you have to do is replace the author, title, abstract,
and text of the paper with your own.

The formatting instructions contained in these style files are
summarized in Sections \ref{gen_inst}, \ref{headings}, and
\ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas)
wide and 9~inches (54~picas) long. The left margin is 1.5~inch
(9~picas).  Use 10~point type with a vertical spacing (leading) of
11~points.  Times New Roman is the preferred typeface throughout, and
will be selected for you by default.  Paragraphs are separated by
\nicefrac{1}{2}~line space (5.5 points), with no indentation.

The paper title should be 17~point, initial caps/lower case, bold,
centered between two horizontal rules. The top rule should be 4~points
thick and the bottom rule should be 1~point thick. Allow
\nicefrac{1}{4}~inch space above and below the title to rules. All
pages should start at 1~inch (6~picas) from the top of the page.

For the final version, authors' names are set in boldface, and each
name is centered above the corresponding address. The lead author's
name is to be listed first (left-most), and the co-authors' names (if
different address) are set to follow. If there is only one co-author,
list both author and co-author side by side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper
nouns), flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the
heading in bold, flush left, and inline with the text, with the
heading followed by 1\,em of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.
Citations may be author/year or numeric, as long as you maintain
internal consistency.  As to the format of the references themselves,
any style is acceptable as long as it is used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations
appropriate for use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may
add the following before loading the \verb+nips_2018+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add
the optional argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{nips_2018}
\end{verbatim}

As submission is double blind, refer to your own published work in the
third person. That is, use ``In the previous work of Jones et
al.\ [4],'' not ``In our previous work [4].'' If you cite your other
papers that are not widely available (e.g., a journal paper under
review), use anonymous author names in the citation, e.g., an author
of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote,
indicate footnotes with a number\footnote{Sample of the first
  footnote.} in the text. Place the footnotes at the bottom of the
page on which they appear.  Precede the footnote with a horizontal
rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction. The figure number and caption
always appear after the figure. Place one line space before the figure
caption and one line space after the figure. The figure caption should
be lower case (except for first word and proper nouns); figures are
numbered consecutively.

You may use color figures.  However, it is best for the figure
captions and the paper body to be legible if the paper is printed in
either black/white or in color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table
number and title always appear before the table.  See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical
  rules.} We strongly suggest the use of the \verb+booktabs+ package,
which allows for typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style
files.  In particular, do not modify the width or length of the
rectangle the text should fit into, and do not change font sizes
(except perhaps in the \textbf{References} section; see below). Please
note that pages should be numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and
not, for example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file
must only contain Type 1 or Embedded TrueType fonts. Here are a few
instructions to achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader,
  select the menu Files$>$Document Properties$>$Fonts and select Show
  All Fonts. You can also use the program \verb+pdffonts+ which comes
  with \verb+xpdf+ and is available out-of-the-box on most Linux
  machines.

\item The IEEE has recommendations for generating PDF files whose
  fonts are also acceptable for NIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap
  fonts.  Use "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You
  should use the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or
\verb+\mathbb{C}+ for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You
can also use the following workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the
\verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we
will ask you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always
specify the figure width as a multiple of the line width as in the
example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly
hyphenate a line. Please give LaTeX hyphenation hints using the
\verb+\-+ command when necessary.

\subsubsection*{Acknowledgments}

Use unnumbered third level headings for the acknowledgments. All
acknowledgments go at the end of the paper. Do not include
acknowledgments in the anonymized submission, only in the final paper.

\section*{References}

References follow the acknowledgments. Use unnumbered first-level
heading for the references. Any choice of citation style is acceptable
as long as you are consistent. It is permissible to reduce the font
size to \verb+small+ (9 point) when listing the references. {\bf
  Remember that you can use more than eight pages as long as the
  additional pages contain \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
  Exploring Realistic Neural Models with the GEneral NEural SImulation
  System.}  New York: TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
learning and recall at excitatory recurrent synapses and cholinergic
modulation in rat hippocampal region CA3. {\it Journal of
  Neuroscience} {\bf 15}(7):5249-5262.

==> result_table.tex <==
\begin{table*}[htb]
	\centering
	\small
	\caption{Edge locality (percentage of uncut edges) computed by various algorithms; 
		$\eps_v$, $\eps_e$ refer to the resulting vertex and degree imbalance, respectively.}
	\begin{tabular}{lrrrrr}
		\toprule
		\multicolumn{1}{c}{Graph}
		& \multicolumn{1}{c}{\algnameshort} %
		& \multicolumn{1}{c}{Hash}
		& \multicolumn{1}{c}{SHP}
		& \multicolumn{1}{c}{Spinner}
		& \multicolumn{1}{c}{LP}  \\
		& & & \multicolumn{1}{c}{\cite{SH16,KKPPSAP17}} & \multicolumn{1}{c}{\cite{MLLS17}} & \multicolumn{1}{c}{\cite{UB13,MSS14}} \\
		\midrule
		\texttt{FB2.5B-2}
		& $80.89$ & $50.00$ & $89.39$ & $85.94$ & $65.66$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.10$ & $\eps_v=1.11$ & $\eps_v=1.00$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.01$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB2.5B-16}
		& $48.39$ & $6.25$ & $60.62$ & $67.78$ & $25.42$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.50$ & $\eps_v=1.40$ & $\eps_v=1.02$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB2.5B-128}
		& $15.10$ & $0.78$ & $44.76$ & $49.42$ & $13.01$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.82$ & $\eps_v=3.12$ & $\eps_v=1.03$ \\
		& $\eps_e=1.01$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.04$ & $\eps_e=1.02$ \\
		\midrule
		\midrule
		\texttt{FB55B-2}
		& $80.33$ & $50.00$ & $86.57$ & $85.78$ & $70.24$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.08$ & $\eps_v=1.05$ & $\eps_v=1.01$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB55B-16}
		& $50.57$ & $6.25$ & $66.62$ & $68.47$ & $35.35$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.12$ & $\eps_v=1.35$ & $\eps_v=1.01$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_v=1.00$ \\
		\midrule
		\texttt{FB55B-128}
		& $?$ & $0.78$ & $54.00$ & $58.35$ & $21.75$ \\
		& $\eps_v=$ & $\eps_v=1.00$ & $\eps_v=1.57$ & $\eps_v=1.65$ & $\eps_v=1.02$ \\
		& $\eps_e=$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_e=1.03$ \\
		\midrule
		\midrule
		\texttt{FB80B-2}
		& $81.53$ & $50.00$ & $91.75$ & $86.49$ & $71.75$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.05$ & $\eps_v=1.08$ & $\eps_v=1.00$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.02$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB80B-16}
		& $50.07$ & $6.25$ & $67.81$ & $70.40$ & $37.16$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.12$ & $\eps_v=1.17$ & $\eps_v=1.01$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.04$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB80B-128}
		& $32.38$ & $0.78$ & $56.46$ & $60.76$ & $23.03$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.40$ & $\eps_v=1.51$ & $\eps_v=1.02$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_e=1.02$ \\
		\midrule
		\midrule
		\texttt{FB400B-2}
		& $76.18$ & $50.00$ & $91.38$ & $92.72$ & $73.58$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.05$ & $\eps_v=1.02$ & $\eps_v=1.00$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.01$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB400B-16}
		& $52.10$ & $6.25$ & $76.5$ & $79.28$ & $43.19$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.12$ & $\eps_v=1.22$ & $\eps_v=1.01$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB400B-128}
		& $?$ & $0.78$ & $58.59$ & $66.37$ & $29.12$ \\
		& $\eps_v=$ & $\eps_v=1.00$ & $\eps_v=1.23$ & $\eps_v=1.80$ & $\eps_v=1.03$ \\
		& $\eps_e=$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.05$ & $\eps_e=1.00$ \\
		\midrule
		\midrule
		\texttt{FB800B-2}
		& $85.87$ & $50.00$ & $93.09$ & $?$ & $72.32$ \\
		& $\eps_v=1.00$ & $\eps_v=1.00$ & $\eps_v=1.01$ & $\eps_v=$ & $\eps_v=1.00$ \\
		& $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB800B-16}
		& $?$ & $6.25$ & $73.17$ & $?$ & $41.75$ \\
		& $\eps_v=$ & $\eps_v=1.00$ & $\eps_v=1.29$ & $\eps_v=$ & $\eps_v=1.01$ \\
		& $\eps_e=$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=$ & $\eps_e=1.00$ \\
		\midrule
		\texttt{FB800B-128}
		& $?$ & $0.78$ & $55.36$ & $?$ & $?$ \\
		& $\eps_v=$ & $\eps_v=1.00$ & $\eps_v=1.31$ & $\eps_v=$ & $\eps_v=$ \\
		& $\eps_e=$ & $\eps_e=1.00$ & $\eps_e=1.00$ & $\eps_e=$ & $\eps_e=$ \\
		\bottomrule
	\end{tabular}
	\label{table:2d_large}
\end{table*}




